Disentangled Representations from Non-Disentangled Models

Constructing disentangled representations is known to be a difficult task, especially in the unsupervised scenario. The dominating paradigm of unsupervised disentanglement is currently to train a generative model that separates different factors of variation in its latent space. This separation is typically enforced by training with specific regularization terms in the model's objective function. These terms, however, introduce additional hyperparameters responsible for the trade-off between disentanglement and generation quality. While tuning these hyperparameters is crucial for proper disentanglement, it is often unclear how to tune them without external supervision. This paper investigates an alternative route to disentangled representations. Namely, we propose to extract such representations from the state-of-the-art generative models trained without disentangling terms in their objectives. This paradigm of post hoc disentanglement employs little or no hyperparameters when learning representations while achieving results on par with existing state-of-the-art, as shown by comparison in terms of established disentanglement metrics, fairness, and the abstract reasoning task. All our code and models are publicly available.

==> tables/isaac.tex <==
\begin{table}
\centering
\footnotesize\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{l|c|c}
        \hline
         Methods & FID $\downarrow$ & MIG $\uparrow$ \\
         \hline
          $\beta$-VAE & 122.6 $\pm$ 2.0 & 0.231 $\pm$ 0.068 \\
          FactorVAE & 305.8 $\pm$ 142.1 & 0.245 $\pm$ 0.034 \\
          $\beta$-TCVAE & 155.4 $\pm$ 13.6 & 0.216 $\pm$ 0.074 \\
          InfoGAN-CR & 80.72 $\pm$ 30.79 & 0.342 $\pm$ 0.139 \\
        \hline
       Info-StyleGAN*  & 8.10 $\pm$ 2.25 &  0.404 $\pm$ 0.085 \\
       Info-StyleGAN  & \textbf{2.19} $\pm$ 0.48 & 0.328 $\pm$ 0.057   \\
         \hline
        StyleGAN 2-DS(1) & 7.22 & \textbf{0.408} \\
         \hline
    \end{tabular}
    \vspace{-2pt}
    \caption{\small Comparison of our method with state-of-the art disentanglement approaches on Isaac3D. Numbers for all the methods except ours are taken from \citep{nie2020semi}.
    Info-StyleGAN* represents the smaller version of Info-StyleGAN, in which its number of parameters is similar to that of previous models. We see that the post hoc disentaglement procedure (\textbf{DS(1)}) allows us to obtain disentagled representations of a similar quality.                 
 }
    \label{tab:disent_scores}
\end{table}
